Question Answering through Transfer Learning from Large Fine-grained Supervision Data

We show that the task of question answering (QA) can significantly benefit from the transfer learning of models trained on a different large, fine-grained QA dataset. We achieve the state of the art in two well-studied QA datasets, WikiQA and SemEval-2016 (Task 3A), through a basic transfer learning technique from SQuAD. For WikiQA, our model outperforms the previous best model by more than 8%. We demonstrate that finer supervision provides better guidance for learning lexical and syntactic information than coarser supervision, through quantitative results and visual analysis. We also show that a similar transfer learning procedure achieves the state of the art on an entailment task.

==> 03-data.tex <==
% \subsection{Set up}

\begin{table*}[ht]
\begin{center}
\resizebox{2.1\columnwidth}{!}{
\begin{tabular}{|l|l||l|l|l||l|l|} 
 \hline
 \multicolumn{2}{|c||}{Span-level QA} & \multicolumn{3}{|c||}{Sentence-level QA} &
 \multicolumn{2}{|c|}{RTE}\\
 \hline
 &\multicolumn{1}{|c||}{SQuAD} & &\multicolumn{1}{|c|}{WikiQA} & \multicolumn{1}{|c||}{SemEval-2016} & & \multicolumn{1}{|c|}{SICK} \\
  \hline
\multirow{3}{*}{\textbf{Q}} &Which company made& \multirow{3}{*}{\textbf{Q}}
&&I saw an ad, data entry jobs online. It req-&&
Four kids are \\
&Spectre? & & Who made airbus &
uired we give a fee and they promise fixed& P &
doing backbends\\
&&&&amount every month. Is this a scam? &&
in the park.\\
  \hline
\multirow{5}{*}{\textbf{C}} &
Spectre (2015) is the&\multirow{2}{*}{\textbf{C1}}&
Airbus SAS is an aircraft manufacturing subsi-
& well  probably is so i be more careful if i&&
Four girls are\\
&24th James Bond film&&
diary of EADS, a European aerospace company.
&were u. Why you looking for online jobs & &
doing backbends\\
  \cline{3-5}
&produced by Eon&  \textbf{C2} &
%Airbus began as a consortium of aerospace manufacturers.
Airbus began as an union of aircraft companies.
& SCAM!!!!!!!!!!!!!!!!!!!!!! & H &
and playing\\
  \cline{3-5}
&
Productions. It
&\multirow{2}{*}{\textbf{C3}}
&
%Consolidation of aerospace companies allowed the establish-
Aerospace companies allowed the establishment
& Bcoz i got a baby and iam nt intrested to&&
outdoors.\\ 
&
features  (...)
&&
%ment of a simplified joint-stock company, owned by EADS.
of a joint-stock company, owned by EADS.
&sent him in a day care. thats y iam (...)&& \\
\hline
\textbf{A} & Eon Productions & \textbf{A} & C1(Y), C2(N), C3(N) & C1(Good), C2(Good), C3(Bad) && Entailment \\
\hline
\end{tabular}
}
\end{center}
\caption{\small Examples of question-context pairs from QA datasets (SQuAD, WikiQA, SemEval-2016 Task3) and premise-hypothesis pair from Recognizing Textual Entailment(RTE) dataset (SICK). \textbf{Q} indicates question, \textbf{C} indicates context, \textbf{A} indicates answer, \textbf{P} indicates premise and \textbf{H} indicates hypothesis. While SQuAD, a span-level QA dataset, requires one to specify the answer span in the context, the other two sentence-level QA datasets require one to choose relevant sentences from the candidates. RT dataset requires one to classify each P-H pair to one of Entailment, Neutral, or Contradiction.}
\label{tab:data}
\end{table*}


 %(Question Id of SemEval in the example : Q318\textunderscore R52)

% Our system is based on BiDAF model from \citep{bidaf}. 
% BiDAF model can be described by the following three steps:
% {\bf (a)} Embed Step consisting character embed layer, word embed layer, and phrase embed layer.
% {\bf (b)} Attention step consisting attention flow from context to question and from question to context.
% {\bf (c)} Output step consisting modelling layer of 2 LSTMs and output layer.

% talk about SQuAD, WikiQA, SemEval
% SQuAD -> MCQA (SQuAD-MC)



We first briefly describe three QA datasets and one non-QA dataset to be used for the experiments in this paper.
Refer to Table~\ref{tab:data} to see an example for each dataset.

\paragraph{SQuAD} (Stanford Question Answering Dataset)~\cite{rajpurkar2016squad} is a recently released, popular span-based QA dataset, containing 100k/10k train/dev examples. Each example in the dataset is a pair of context paragraph extracted from Wikipedia and a question created by a human, and the answer is a span in the context.


\paragraph{WikiQA}~\cite{yang2015wikiqa} is an example of sentence-level QA dataset, containing 1.9k/0.3k train/dev answerable examples.
Each example consists of a real user's Bing query and a snippet of a Wikipedia article retrieved by Bing. The answer to the query is one of the sentences in the snippet that provides sufficient information. 

\paragraph{SemEval 2016}~\cite{alessandromoschitti2016semeval} is another example of sentence-level QA dataset, containing 1.8k/0.2k/0.3k train/dev/test examples.
Each example consists of a community question by a user and other users' comments (answer candidates) on it. 
The task is to select the comments that correctly answer the question.

\paragraph{SICK} \cite{marelli2014sick} is a dataset for recognizing textual entailment (RTE).
SNLI \cite{bowman2015large} is ...
More explanations will go here...

\vspace{2mm}

Lastly, we introduce one more dataset, \emph{SQuAD-C}, for which we modified SQuAD to create a same-size sentence-level QA dataset.
We split the context paragraph into sentences, and we formulate the task as choosing the sentence that contains the answer, making SQuAD more similar to WikiQA and SemEval 2016. This enables us to make a fair comparison between span-supervised and sentence-supervised QA.

% In our experiments, we perform transfer learning from SQuAD and SQuAD-MC to WikiQA and SemEval 2016.
% We first train models on SQuAD and SQuAD-MC, and we describe the model architectures in Section~\ref{subsec:model}.
% Then we describe the details of transfer learning, elaborating how we initialize WikiQA and SemEval 2016 model weights with the pretrained models.
% In Section~\ref{sec:exp}, we thoroughly compare between transfer learning with SQuAD and SQuAD-MC, and provide visual analysis of the resulting models' learning ability. 






==> 13-app-D.tex <==
\begin{table}[ht]
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|} 
 \hline
 Question & Id & WO-P & W-P \\ 
 \hline
what are circumpolar constellations & 1 &  N &  Y \\ 
what is homebrew for wii & 1 &  Y &  Y \\ 
who was mr big on sex and the city & 1 &  Y &  Y \\ 
who is flo from progressive & 1 &  N &  Y \\ 
when did spongebob first air & 1 &  N &  Y \\ 
What is the prostate for ? & 1 &  Y &  Y \\ 
what is doxycycline hyclate used for & 1 &  Y &  Y \\ 
what is a letterbox movie & 1 &  N &  Y \\ 
what is the la tour de france & 1 &  Y &  Y \\ 
what are layers of the ionosphere & 1 &  N &  Y \\ 
where was martin luther king shot ? & 1 &  Y &  Y \\ 
what is a neuro tract & 1 &  Y &  Y \\ 
where is the brisket from & 1 &  Y &  Y \\ 
what food is in afghan & 1 &  Y &  Y \\ 
what is a wwII theater & 1 &  Y &  Y \\ 
what is in a hot toddy & 1 &  Y &  Y \\ 
when does the royal standard fly ? & 1 &  N &  Y \\ 
who is st patty ? & 1 &  Y &  Y \\ 
how does interlibrary loan work & 1 &  Y &  Y \\ 
who first synthesized heroin & 1 &  Y &  Y \\ 
where is humboldt ks & 1 &  Y &  Y \\ 
what is the oath of allegiance of the united states & 1 &  Y &  Y \\ 
WHAT IS PARESTHESIAS OF HANDS & 1 &  Y &  Y \\ 
what is a newsgroup message & 1 &  Y &  Y \\ 
who is basketball star antoine walker & 1 &  Y &  Y \\ 
how does a dim sum restaurant work & 1 &  Y &  Y \\ 
what is the color puce & 1 &  N &  Y \\ 
what county is bethlehem pa in & 1 &  Y &  Y \\ 
what does righteousness mean & 1 &  Y &  Y \\ 
what is the great basin area & 1 &  Y &  N \\ 
where does a flea live & 1 &  N &  Y \\ 
what is an army specialist & 1 &  Y &  Y \\ 
What are procedure codes terms in coding ? & 1 &  Y &  Y \\ 
where is the sermon on the mount in the bible & 1 &  Y &  Y \\ 
how many mvps has kobe bryant won & 1 &  Y &  Y \\ 
what county is bolingbrook il in ? & 1 &  Y &  Y \\ 
what is in a tequila sunrise ? & 1 &  Y &  Y \\ 
 \hline 
how many days are in a leap year & 2 &  Y &  N \\ 
who played the lead roles in the movie leaving las vegas & 2 &  N &  N \\ 
who did mr bojangles & 2 &  Y &  Y \\ 
what does hair testing show & 2 &  Y &  Y \\ 
where was the first real roller coaster & 2 &  N &  Y \\ 
what are some six sigma tools used & 2 &  N &  Y \\ 
when was How the west was won filmed ? & 2 &  Y &  Y \\ 
what county is coatesville indiana located in & 2 &  Y &  Y \\ 
where was hillary clinton born & 2 &  N &  N \\ 
who sang I want to dance with somebody & 2 &  N &  Y \\ 
when did the movie deep blue sea come out & 2 &  Y &  Y \\ 
who has brad pitt dated & 2 &  N &  N \\ 
what countries did immigrants come from during the immigration & 2 &  N &  Y \\ 
what are some legal uses of meth & 2 &  Y &  N \\ 
what year was the eiffel tower made & 2 &  N &  Y \\ 
when did ww1 end ? & 2 &  Y &  Y \\ 
who wrote the song for star wars & 2 &  N &  Y \\ 
WHere is a famous alluvial plain & 2 &  Y &  Y \\ 
what are the parts of plant stems ? & 2 &  N &  Y \\ 
Where Elephants Live & 2 &  Y &  N \\ 
where is al jazeera based & 2 &  Y &  Y \\ 
what relates to erosion & 2 &  Y &  Y \\ 
Where does the word baptism come from & 2 &  Y &  Y \\ 
what is the type of democracy in which all citizens have the right to (...) & 2 &  N &  Y \\ 
how many numbers on a credit card & 2 &  N &  Y \\ 
what is the ingredient in mustard & 2 &  N &  Y \\ 
HOW AFRICAN AMERICANS WERE IMMIGRATED TO THE US & 2 &  N &  Y \\ 
what year was christianity introduced to sub-saharan africa & 2 &  Y &  N \\ 
what can be powered by wind & 2 &  Y &  Y \\ 
how are antibodies used in & 2 &  N &  Y \\ 
who set the world record for women for high jump & 2 &  N &  N \\ 
who are all of the jonas brothers & 2 &  N &  N \\ 
how many books are included in the protestant Bible ? & 2 &  Y &  Y \\ 
how many amendments in us & 2 &  Y &  Y \\ 
How long was Mickie James with WWE ? & 2 &  N &  N \\ 
what creates a cloud & 2 &  Y &  Y \\ 
how did women 's role change during the war & 2 &  N &  Y \\ 
who made the matrix & 2 &  N &  Y \\ 
 \hline 
what species is a spider & 3 &  N &  N \\ 
when was Mary Anderson born & 3 &  Y &  Y \\ 
what was the first year of kentucky derby & 3 &  Y &  N \\ 
what is the latest season of psych & 3 &  N &  Y \\ 
when did proof die & 3 &  Y &  Y \\ 
what year did isaac newton die & 3 &  Y &  Y \\ 
 \hline 
when did texas become a state & 4 &  N &  N \\ 
How much did Waterboy grossed & 4 &  N &  Y \\ 
what day is 2011 super bowl ? & 4 &  Y &  Y \\ 
what can sql 2005 do & 4 &  Y &  N \\ 
what is brown flax & 4 &  N &  N \\ 
what is the function of the liver & 4 &  N &  N \\ 
what county is jacksonville florida in & 4 &  Y &  N \\ 
where in oregon is albany & 4 &  Y &  Y \\ 
what religion is primary in africa ? & 4 &  N &  N \\ 
what school did Zach Thomas play for before making it in to the NFL & 4 &  N &  Y \\ 
what does s.h.i.e.l.d stand for & 4 &  N &  N \\ 
where is the 2011 mlb all star game location & 4 &  Y &  Y \\ 
where is cougar town filmed & 4 &  Y &  N \\ 
where do the mohawks live & 4 &  Y &  Y \\ 
who is on blink 182 album cover & 4 &  N &  Y \\ 
 \hline 
How Do You Play Spades & 5 &  N &  N \\ 
what were 3 important things that douglas MacArthur did ? & 5 &  N &  N \\ 
 \hline 
how kimberlite pipes form & 6 &  N &  N \\ 
how many members are in the house of representatives & 6 &  N &  N \\  
 \hline 
\end{tabular}
}
\end{center}
\caption{ \small 100 samples from WikiQA. Id indicates category id, and WO-P/W-P means whether the best model without/with pretrain got correct. }
\label{tab:sample-wikiqa}
\end{table}


\begin{table}[ht]
\begin{center}
\fontsize{2}{2}\selectfont
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|} 
 \hline
 Question Id & Id & WO-P  & W-P \\ 
 \hline
Q338\textunderscore R30 & 1 &  Y &  Y \\ 
Q336\textunderscore R13 & 1 &  N &  N \\ 
Q386\textunderscore R19 & 1 &  Y &  Y \\ 
Q325\textunderscore R1 & 1 &  Y &  Y \\ 
Q322\textunderscore R9 & 1 &  Y &  N \\ 
Q373\textunderscore R1 & 1 &  N &  N \\ 
Q335\textunderscore R19 & 1 &  Y &  Y \\ 
Q351\textunderscore R27 & 1 &  Y &  N \\ 
Q372\textunderscore R6 & 1 &  N &  N \\ 
Q381\textunderscore R1 & 1 &  N &  N \\ 
Q345\textunderscore R14 & 1 &  N &  N \\ 
Q379\textunderscore R22 & 1 &  Y &  N \\ 
Q319\textunderscore R40 & 1 &  N &  N \\ 
Q332\textunderscore R15 & 1 &  Y &  Y \\ 
Q355\textunderscore R3 & 1 &  N &  N \\ 
Q330\textunderscore R44 & 1 &  N &  N \\ 
Q340\textunderscore R27 & 1 &  Y &  Y \\ 
Q332\textunderscore R2 & 1 &  Y &  Y \\ 
Q366\textunderscore R53 & 1 &  Y &  Y \\ 
Q330\textunderscore R53 & 1 &  Y &  Y \\ 
Q341\textunderscore R75 & 1 &  N &  N \\ 
Q331\textunderscore R1 & 1 &  Y &  Y \\ 
Q334\textunderscore R1 & 1 &  Y &  Y \\ 
Q350\textunderscore R4 & 1 &  N &  N \\ 
Q330\textunderscore R96 & 1 &  Y &  N \\ 
Q338\textunderscore R27 & 1 &  Y &  Y \\ 
Q346\textunderscore R31 & 1 &  Y &  N \\ 
Q384\textunderscore R46 & 1 &  N &  N \\ 
Q333\textunderscore R27 & 1 &  Y &  N \\ 
\hline
Q326\textunderscore R90 & 2 &  Y &  N \\ 
Q343\textunderscore R11 & 2 &  N &  N \\ 
Q324\textunderscore R5 & 2 &  Y &  N \\ 
Q330\textunderscore R22 & 2 &  N &  N \\ 
Q356\textunderscore R13 & 2 &  Y &  Y \\ 
Q320\textunderscore R1 & 2 &  N &  N \\ 
Q324\textunderscore R21 & 2 &  Y &  Y \\ 
Q363\textunderscore R58 & 2 &  N &  N \\ 
Q385\textunderscore R2 & 2 &  N &  N \\ 
Q366\textunderscore R41 & 2 &  Y &  Y \\ 
Q381\textunderscore R11 & 2 &  Y &  Y \\ 
Q326\textunderscore R3 & 2 &  N &  N \\ 
Q339\textunderscore R42 & 2 &  N &  N \\ 
Q350\textunderscore R15 & 2 &  Y &  Y \\ 
Q365\textunderscore R52 & 2 &  Y &  Y \\ 
Q377\textunderscore R56 & 2 &  Y &  N \\ 
Q354\textunderscore R44 & 2 &  Y &  N \\ 
Q370\textunderscore R1 & 2 &  N &  N \\ 
Q351\textunderscore R11 & 2 &  N &  N \\ 
Q329\textunderscore R21 & 2 &  N &  N \\ 
Q335\textunderscore R9 & 2 &  Y &  N \\ 
Q340\textunderscore R88 & 2 &  Y &  N \\ 
Q385\textunderscore R34 & 2 &  N &  N \\ 
Q319\textunderscore R1 & 2 &  Y &  Y \\ 
Q348\textunderscore R36 & 2 &  N &  N \\ 
Q345\textunderscore R1 & 2 &  N &  N \\ 
Q366\textunderscore R40 & 2 &  Y &  N \\ 
Q347\textunderscore R1 & 2 &  Y &  N \\ 
Q361\textunderscore R22 & 2 &  Y &  N \\ 
Q385\textunderscore R25 & 2 &  N &  N \\ 
Q382\textunderscore R54 & 2 &  N &  N \\ 
Q326\textunderscore R64 & 2 &  Y &  N \\ 
Q377\textunderscore R11 & 2 &  Y &  Y \\ 
Q349\textunderscore R30 & 2 &  Y &  Y \\ 
Q323\textunderscore R4 & 2 &  N &  Y \\ 
Q326\textunderscore R34 & 2 &  Y &  Y \\ 
Q325\textunderscore R56 & 2 &  Y &  Y \\ 
Q341\textunderscore R87 & 2 &  N &  N \\ 
\hline
Q358\textunderscore R50 & 3 &  N &  Y \\ 
Q370\textunderscore R52 & 3 &  Y &  Y \\ 
Q323\textunderscore R12 & 3 &  N &  Y \\ 
Q352\textunderscore R58 & 3 &  Y &  Y \\ 
Q359\textunderscore R38 & 3 &  N &  N \\ 
Q337\textunderscore R36 & 3 &  N &  N \\ 
Q338\textunderscore R34 & 3 &  N &  N \\ 
\hline
Q329\textunderscore R73 & 4 &  Y &  N \\ 
Q341\textunderscore R11 & 4 &  N &  N \\ 
Q344\textunderscore R46 & 4 &  N &  N \\ 
Q387\textunderscore R30 & 4 &  Y &  Y \\ 
Q369\textunderscore R28 & 4 &  N &  Y \\ 
Q375\textunderscore R27 & 4 &  N &  N \\ 
Q345\textunderscore R67 & 4 &  Y &  N \\ 
Q348\textunderscore R34 & 4 &  N &  N \\ 
Q358\textunderscore R52 & 4 &  Y &  Y \\ 
Q348\textunderscore R6 & 4 &  Y &  Y \\ 
Q372\textunderscore R31 & 4 &  Y &  Y \\ 
Q346\textunderscore R2 & 4 &  Y &  Y \\ 
\hline
Q351\textunderscore R12 & 5 &  N &  N \\ 
Q360\textunderscore R42 & 5 &  N &  N \\ 
Q366\textunderscore R24 & 5 &  N &  N \\ 
Q371\textunderscore R42 & 5 &  N &  N \\ 
Q382\textunderscore R23 & 5 &  Y &  N \\ 
Q323\textunderscore R7 & 5 &  N &  N \\ 
Q370\textunderscore R11 & 5 &  N &  N \\ 
Q319\textunderscore R44 & 5 &  Y &  N \\ 
Q372\textunderscore R40 & 5 &  N &  N \\ 
\hline
Q352\textunderscore R64 & 6 &  N &  N \\ 
Q367\textunderscore R1 & 6 &  Y &  N \\ 
Q337\textunderscore R16 & 6 &  Y &  N \\ 
Q323\textunderscore R10 & 6 &  N &  Y \\ 
Q350\textunderscore R26 & 6 &  N &  N \\ 
\hline



\end{tabular}
}
\end{center}
\caption{ \small 100 samples from Semeval-2016. Id indicates category id, and WO-P/W-P means whether the best model without/with pretrain got correct.  }
\label{tab:sample-semeval}
\end{table}

